Incident-aware Duplicate Ticket Aggregation for Cloud Systems

In cloud systems, incidents are potential threats to customer satisfaction and business revenue. When customers are affected by incidents, they often request customer support service (CSS) from the cloud provider by submitting a support ticket. Many tickets could be duplicate as they are reported in a distributed and uncoordinated manner. Thus, aggregating such duplicate tickets is essential for efficient ticket management. Previous studies mainly rely on tickets' textual similarity to detect duplication; however, duplicate tickets in a cloud system could carry semantically different descriptions due to the complex service dependency of the cloud system. To tackle this problem, we propose iPACK, an incident-aware method for aggregating duplicate tickets by fusing the failure information between the customer side (i.e., tickets) and the cloud side (i.e., incidents). We extensively evaluate iPACK on three datasets collected from the production environment of a large-scale cloud platform, Azure. The experimental results show that iPACK can precisely and comprehensively aggregate duplicate tickets, achieving an F1 score of 0.871 ~ 0.935 and outperforming state-of-the-art methods by 12.4% ~ 31.2%.

==> Content/discussion.tex <==
\section{Discussion}
\subsection{customer-side problems}

==> Content/empirical_study.tex <==
\subsection{Empirical Study}
\label{sec: empirical_study}
% \zb{from the current intro, it is not very clear why we study these three specific questions in the empirical study. also, in each part, need to mention how the findings guide the design of the approach}
To understand the impact of cloud incidents on support tickets and alerts in a real production environment, we conduct the following empirical study based on two years of real-world data (01/01/2020 to 01/01/2022) in \cloud.
Due to confidential issues, we apply normalization to the data.
Particularly, we aim to answer the following research questions (RQ).

% How different monitors are triggered by an incident? 

\begin{itemize}[leftmargin=*, topsep=0pt]
    \item \textbf{RQ1}: How many services can be affected by an incident?
    % \item \textbf{RQ2}: \jy{What is the cost of handling tickets?}
    % \item \textbf{RQ2}: During incidents, are there any co-occurrence patterns among alerts?
    \item \textbf{RQ3}: \jy{What correlations do tickets and alerts exhibit, if any?}
\end{itemize}

% \begin{figure}[t]
%   \centering
%   \mbox{
% %   Impact of alerts with different levels of severity
%      \subfigure[Number of services impacted by an incident with varying severity\label{fig: cross-service-alerts}]{\includegraphics[width=0.45\columnwidth]{Figures/num_service_affcted.pdf}}\quad
    
%     \subfigure[Distribution of Time to close a ticket.
%     \label{fig: ttc}]{\includegraphics[width=0.45\columnwidth]{Figures/sr_handle_time.pdf}}\quad
%     }
% \mbox{
%     \subfigure[Distribution of time interval between alert firing and tickets submission.
%     % \jy{replace with the bar chart}
%     \label{fig: time_interval}]
%     {\includegraphics[width=0.45\columnwidth]{Figures/time_interval.pdf}}
    
%     \subfigure[Distribution of events related to different number of topics.  \label{fig: monitor_affect_topics}]{\includegraphics[width=0.45\columnwidth]{Figures/event_affect_topics.pdf}}\quad
%   }
%   \caption{Empirical analysis results on the ticket and alert data in \cloud.}
%   \label{main figure label}
% \end{figure}


% \zb{dont quite get the purpose of this empirical study. use more plain and concrete language. for audience, words like ``relation'' and ``connection'' are hard to understand.}


\subsubsection{\textbf{RQ1} Cross-Service Impact of Incidents}
% \jy{emphasize the impact of high-level incidents}
In the workflow of incident processing, engineers analyze and mark which services are affected for each incident. 
Based on this annotated data, we calculate the CDF (cumulative distribution function) of the number of services impacted by an incident. We plot the figure by varying the incident severity.
As shown in figure~\ref{fig: cross-service-alerts}, more severe incidents tend to affect more services. Nearly 70\% high-severity incidents affect at least two services.
In contrast, around 70\% of medium-level incidents and 80\% low-level incidents only affect one service, but they are still possible to affect more than one services.

Although customers of a specific service may experience similar problems when they are affected by an incident, they could write different free texts to describe the symptoms.
% \zb{this is mentioned in intro}\slhe{emphasize again?}\zb{lack transition, added}
The issue is compounded by the fact that incidents with cross-service impact are common. It is more challenging to identify duplicate tickets, because customers from different services tend to perceive distinct failure symptoms, leading to tickets with dissimilar semantics.
% Especially, an incident can finally lead to tens of tickets to $\sim$200 duplicate tickets.


\begin{tcolorbox}
[colback=black!10,%gray background
colframe=black!10,% black frame colour
width=1\linewidth,% Use 5cm total width,
arc=0mm, auto outer arc,
%   title=Findings
%   borderline={1pt}{1pt}
box align=center,
left = 0pt,
right = 0pt,
top=0pt,
bottom=0pt,
% halign=center,
% valign=center,
]
\textbf{Finding 1}
Cloud incidents can produce cross-service impacts.
Customers using the impacted services can submit quite different tickets, which makes it challenging to identify duplicate tickets.
\end{tcolorbox}

% \subsubsection{\textbf{RQ2}
% Co-occurrence of Alerts During Incidents.}
% % \zb{can the co-occurrence of components implies the relation of alerts? one component may associate with multiple monitors?}
% As introduced in Section~\ref{sec: bg_alert_and_tickets}, alerts are generated by monitors that engineers deploy to report various anomalies in cloud systems. During postmortem analysis of an incident, engineers will label the set of alerts that are triggered by the incident. In this RQ, we aim to understand whether there are some types of alerts that are constantly reported together in multiple incidents. If cases are found, we are allowed to mine frequent patterns of alert co-occurrence accordingly.

% We study historical incidents and the alerts reported along with each incident within the recent two years. We first aggregate alerts describing the same issue as an event (see Section~\ref{sec: agg}). Then, we enumerate all pairs of different events in each incident. Finally, we count the occurrence of all event pairs in different incidents. 
% The results are shown in Figure~\ref{fig: comp_co_occ}, which is the histogram of the occurrence number of different event pairs. For example, the first bar indicates that $\sim$10,000 pairs of events do not frequently appear, i.e., in less than 30 incidents. 
% % \llq{not very clear, need some descriptions about how to interpret this figure.}
% However, there are a considerable number of event pairs that show up frequently, i.e., in at least 30 incidents (shown by the remaining bars).
% The large number of event pairs with a high occurrence rate indicates the strong correlation among certain events in cloud systems. 
% It is worth noting that we also find a similar distribution of service pairs that are often impacted by incidents. We omit the concrete figure due to space limitations.
% % As monitors will fire alert when the components are concurrently impacted by an incident, we are allowed to mine frequent alert co-occurrence patterns accordingly.


% % Co-occurrence of Components During an Incident.}

% % \zb{why not just study the co-occurrence of alerts (or events)? ``component'' is not well-defined, can be very vague.}
% % In addition to services, we take a close look at the fine-grained components affected by an incident. As introduced in Section~\ref{sec: bg_alert_and_tickets}, components often represents a specific functionality or feature where the monitor is configured. In this RQ, we aim to understand whether some components are concurrently impacted in multiple incidents. If yes, it points out the potential to learn the alert co-occurrence pattern from historical data since the alert is created on top of the component.

% % We studied historical incidents ($\sim$100,000) and the components affected by these incidents.
% % We combine each two components in an incident as pairs and count the co-occurrence of the pairs in different incidents. 
% % The results are shown in Figure~\ref{fig: comp_co_occ}.
% % We can find that $\sim$10,000 pairs of components are not frequently impacted together (i.e., co-occur in less than 30 incidents as shown in the first bar of Figure~\ref{fig: comp_co_occ}). 
% % However, there are considerable numbers of component pairs frequently impacted in the same incidents, namely, the pairs show in at least 30 incidents (shows in the remaining bars).
% % The large number of component co-occurrence indicates the strong dependency of different components in the cloud systems. 
% % It is worth noting that we also find a similar distribution for service pairs, and we omit the concrete figure to save space.
% % As monitors will fire alert when the components are concurrently impacted by an incident, we are allowed to mine frequent alert co-occurrence patterns accordingly.


% \begin{tcolorbox}
% [colback=black!10,%gray background
% colframe=black!10,% black frame colour
% width=1\linewidth,% Use 5cm total width,
% arc=0mm, auto outer arc,
% %   title=Findings
% %   borderline={1pt}{1pt}
% box align=center,
% left = 0pt,
% right = 0pt,
% top=0pt,
% bottom=0pt,
% % halign=center,
% % valign=center,
% ]
% \textbf{Finding 2}
% % Different functionalities are dependent on each other in cloud systems with a hierarchical structure.
% When incidents happen, a considerable number of events (i.e., alerts describing the same issue) are frequently reported together, which motivates us to mine the frequent co-occurrence patterns between alerts. 
% \end{tcolorbox}

\subsubsection{\textbf{RQ2} Cost of Handling Tickets}
\label{sec: empirical_sr_cost}
See Figure~\ref{fig: ttc}. May be meaningless after normalization.

% \subsubsection{\textbf{RQ3} Correlation Between Alerts and Tickets}
% \label{sec: empirical_feasibility}

% In CSS team's daily workflow, if engineers find one ticket is caused by a cloud-side incident,
% % \zb{what do you mean tickets are caused by alerts? aren't they caused by incidents?}\slhe{revised}
% they will manually annotate the alerts that are responsible for the ticket. These responsible alerts indicate the cloud-side issues that cause the problems described in the ticket.
% % \slhe{should add the ``related alert'' to 2.1 and the example to explain where the label comes from}
% % \jy{in the figure? not every ticket owns this.}
% % are required to record the resolution results to close a ticket in their workflow.
% Based on the manual annotation, we first calculate the time difference between the ticket and the earliest alert.
% Figure~\ref{fig: time_interval} shows that the majority of responsible alerts (around 89\%) happen before a ticket is submitted, mostly 0-12 hours earlier. This implies the chance to correlate alerts to tickets when tickets are received.
% % However, there are some alerts created later than the related ticket is submitted. We suspect the reason as follows: although some customers have been impacted by a cloud side problem, but the monitor does not fire an alert until the metric reaches the alerting threshold. 

% Then, based on the same dataset, we study if a specific type of alert (i.e., event) could be correlated to tickets with a specific symptom, which is indicated by the \textit{topic} field. To this end, we count the number of different ticket topics that each event could be responsible for.
% Figure~\ref{fig: monitor_affect_topics} shows that 55\% of events can be linked to one ticket topic (as shown in the leftmost bar with range $[0, 2)$).
% This shows that these alerts are dedicated to monitor the specific issues for customers, indicating a strong correlation between alerts and tickets.
% However, there are still 45\% of events that can be mapped to more than two kinds of ticket topics.
% Therefore, we cannot rely solely on the mapping between event and ticket's topic to decide the relation between alerts and tickets, leaving spaces for involving more features to achieve better performance (Section~\ref{sec: ticket-event-correlation}).



% % This is mainly caused by the sensitivity of threshold setting of an alert. Namely, the corresponding monitor does not fire an incident yet when the monitored object only slightly turns unhealthy but has impacted some customers.
% % In spite of this, alerts that are related to a ticket can be potentially found inside the cloud systems in most cases.


% % Then, based on the same dataset, we study if a specific kind of alert could correspond to tickets with a specific symptom (i.e., topics). To this end, we count the number of different ticket topics \llq{use num of topics instead of tickets is for privacy concern? the objective is to reduce duplicated tickets. but no result supports this problem yet.} that each alert monitor could correspond.
% % \zb{what do you mean by ``correspond to''? they have some keywords in common, or this is done manually?} \slhe{revised, plz check}
% % If so, we are able to automatically correlate alerts and the resulting tickets via data-driven approaches. % accordingly.
% % Figure~\ref{fig: monitor_affect_topics} shows that 55\% alerts that fired from a particular monitor can only link to a specific topic of tickets (as shown in the left most bar with range $[0, 2)$). 
% % This implies that these monitors are precisely configured to monitor specific functionalities for customers.
% % However, there are still 45\% monitors that fire alerts corresponding to more than two kinds of topics of tickets.
% % Therefore, we cannot decide which tickets are affected by an incident by relying on monitors only, leaving spaces for involving more features of tickets and alerts to achieve so (Section~\ref{sec: ticket-event-correlation}).
% % \jy{change}
% % The same symptom of a problem from the user-side can be caused by problems from various root-cause services in cloud systems, namely, the relations between user-side symptoms and cloud-side problems are dynamic.
% % Based on support engineers' diagnosis histories of support tickets, we analyse the ratio of root-cause services of different symptoms (i.e., topics).  
% % The results are shown in Figure~\ref{}
% % A topic (symptom) is caused by one responsible service in most cases. Usually, the responsible service is directly used by the customer, which is a directly related service; However, different services other than the directly related services can still cause the same problem of a customer. For instance, mostly, S3 is responsible for these ST of topic T3. Nevertheless, other different services can also finally lead to T3, e.g., S6 and S8. 

% % \textbf{Volume Number Change During an Outage.} 
% % \jy{change}
% % % \jy{emphasize generalization}
% % We show a real cloud incident that affected different services\footnote{The public link to this incident is temporarily masked due to double-blind policy.}.
% % As shown in Figure~\ref{fig: ticket_num_change}, the incident happens at around 07/07/2021 21:00 UTC. 
% % S1 to S5 are five major services affected by this incident in \cloud.
% % We can see that the volume of tickets reported from S1 shows a clear increase at 09:00 the next day, when the engineers started to work and found their services are affected.
% % In contrast, we do not observe a significant burst in services S2-S5. The reason is that these services have customers less than S1, thus tickets complaining about the incident are more like to be buried in daily tickets.
% % However, if we sum the numbers of tickets of these affected services, we can observe a significantly higher volume from 07:00 to 12:00 before the incident is resolved.
% % This shows that these services are actually affected by the same incident simultaneously, thus the tickets in these service should be grouped together to handle in a batch manner.

% % We select six services that report the most incidents in \cloud, i.e. \jy{}, then collect the incidents they produced from 01/01/2021 to 31/12/2021.
% % We compute the average numbers of incidents the services reported per day.
% % Figure~\ref{fig: many_alerts_per_day} show that S1 reports more than ten thousands incidents per day and S6 reports the minimal number of incidents but still can possibly overwhelm the engineers with nearly two thousand incidents.


% % Figure~\ref{fig: same_topic_to_rootcauses} A topic (symptom) is caused by one responsible service in most cases. Usually, the responsible service is directly used by the customer, which is a directly related service; However, different services other than the directly related services can still cause the same problem of a customer. For instance, mostly, S3 is responsible for these ST of topic T3. Nevertheless, other different services can also finally lead to T3, e.g., S6 and S8. 


% % Engineers need twice of time to resolve the STs that are caused by problems in \cloud than the STs caused by customer-side problems.


% \begin{tcolorbox}
% [colback=black!10,%gray background
% colframe=black!10,% black frame colour
% width=1\linewidth,% Use 5cm total width,
% arc=0mm, auto outer arc,
% %   title=Findings
% %   borderline={1pt}{1pt}
% box align=center,
% left = 0pt,
% right = 0pt,
% top=0pt,
% bottom=0pt,
% % halign=center,
% % valign=center,
% ]
% % (1) Cloud incidents can product cross-service impact.
% % Especially, nearly 70\% high-severity incidents affect more than two services.
% % The customers using the impacted services can submit quite different tickets, which makes it challenging to group duplicate tickets.
% % (2) Different functionalities are dependent on each other in cloud systems with a hierarchical structure. Therefore, when an incident happens, a considerable number of monitor pairs can frequently fire alerts simultaneously, which motivates us to mine the relations between alert based on such frequent patterns. 
% \textbf{Finding 3}
% Most alerts (89\%) can be fired before customers submit the corresponding tickets.
% % Consequently, we are able to find the potential alert that is related to a ticket.
% In addition, while there is a rough mapping between alerts and tickets, more features are required to correlate them more accurately.
% \end{tcolorbox}




% indicate one specific customer's symptoms

% \begin{flushleft}
% \begin{tabular}{|>{\raggedright}p{0.95\columnwidth}|}
% \noalign{\vskip4pt}
% \hline 
% \textsc{Summary of findings}. 
% % \jy{cross-service impact, higher->more service impacted}
% (1) Cloud incidents can product cross-service impact.
% Especially, nearly 70\% high-severity incidents affect more than two services.
% The customers using the impacted services can submit quite different tickets, which makes it challenging to group duplicate tickets.

% (2) Different functionalities are dependent on each other in cloud systems with a hierarchical structure. Therefore, when an incident happens, a considerable number of monitor pairs can frequently fire alerts simultaneously, which motivates us to mine the relations between alert based on such frequent patterns. 
% (3) Most alerts (89\%) can be early detected before customers submit corresponding tickets. Consequently, we are able to find the potential alert that is related to a ticket.
% In addition, 55\% monitors are precise enough to indicate one specific customer's symptoms. 
% Therefore, besides the monitors that firing the alert, we should also consider specific features (e.g., title) of both tickets and alerts to correlate them.

% \tabularnewline
% \hline 
% \multicolumn{1}{>{\raggedright}p{0.95\columnwidth}}{}\tabularnewline
% \noalign{\vskip-6pt}
% \end{tabular}
% \par\end{flushleft}
